Benchmarking Reinforcement Learning Techniques for Autonomous Navigation

Deep reinforcement learning (RL) has brought many successes for autonomous robot navigation. However, there still exists important limitations that prevent real-world use of RL-based navigation systems. For example, most learning approaches lack safety guarantees; and learned navigation systems may not generalize well to unseen environments. Despite a variety of recent learning techniques to tackle these challenges in general, a lack of an open-source benchmark and reproducible learning methods specifically for autonomous navigation makes it difficult for roboticists to choose what learning methods to use for their mobile robots and for learning researchers to identify current shortcomings of general learning methods for autonomous navigation. In this paper, we identify four major desiderata of applying deep RL approaches for autonomous navigation: (D1) reasoning under uncertainty, (D2) safety, (D3) learning from limited trial-and-error data, and (D4) generalization to diverse and novel environments. Then, we explore four major classes of learning techniques with the purpose of achieving one or more of the four desiderata: memory-based neural network architectures (D1), safe RL (D2), model-based RL (D2, D3), and domain randomization (D4). By deploying these learning techniques in a new open-source large-scale navigation benchmark and real-world environments, we perform a comprehensive study aimed at establishing to what extent can these techniques achieve these desiderata for RL-based navigation systems.

==> contents/related.tex <==
\section{Related Work}
\rebuttal{
Our proposed benchmark differs from existing benchmarks in three aspects: (1) \textbf{high-fidelity physics}: the navigation tasks are simulated by Gazebo~\cite{koenig2004design}, which is based on realistic physical dynamics and therefore tests motion planners that directly produce low-level motion commands, i.e., linear and angular velocies, in contrast to high-level instructions such as turn left, turn right, move forward \cite{zhu2017target, harries2019mazeexplorer}. In other words, we focus on ``how to navigate" (motion planning), instead of ``where to navigate" (path planning); (2) \textbf{ROS integration}: our benchmark is based on ROS \cite{ros}, which allows seamless transfer of a navigation method developed and benchmarked in simulation directly onto a physical robot with little (if any) effort; and (3) \textbf{collision-free navigation}: the benchmark includes both static and dynamic environments, and requires \emph{collision-free} navigation, whereas other benchmarks assume that either collisions are possible \cite{harries2019mazeexplorer} or collision-avoidance will be addressed by other low-level controllers out of the scope of the benchmark \cite{zhu2017target}. A special case is the photo-realistic interactive Gibson benchmark by Xia et. al.~\cite{xia2020interactive}, which intentionally allows physical interaction with objects (e.g., pushing) and therefore pose no challenges to the collision-avoidance system. All these three features of our benchmark facilitate a direct transfer of a navigation system to the real world, and the benchmarked performance is expected to be more consistent between simulation and the real world than other benchmarks with different focuses.}

%\rebuttal{
%In the remaining part of this section, we discuss existing navigation benchmarks and highlight the differences in terms of the three aspects. First, the interactive Gibson benchmark by Xia et. al.~\cite{xia2020interactive} focused on photo-realistic visual navigation in household environments, where physical interaction with objects (e.g., pushing) is allowed to reach the goal. Therefore, no challenges are posed to the collision-avoidance system. In our benchmark, we focus on completely collision-free navigation even if obstacles are very close to the robot. Moreover, Marchesini et. al.~\cite{marchesini2021benchmarking} presented a benchmark for aquatic navigation of water vehicles, whereas our benchmark focuses on ground navigation in obstacle occupied spaces. Another navigation benchmark, Mazeexplorer~\cite{harries2019mazeexplorer}, is based on the 3D first-person game Doom and open source environment VizDoom, which does not test low-level motion commands and obstacle avoidance.
%}
